Vid2Sim: Realistic and Interactive Simulation from Video for Urban Navigation

Sim-to-real gap has long posed a significant challenge for robot learning in simulation, preventing the deployment of learned models in the real world. Previous work has primarily focused on domain randomization and system identification to mitigate this gap. However, these methods are often limited by the inherent constraints of the simulation and graphics engines. In this work, we propose Vid2Sim, a novel framework that effectively bridges the sim2real gap through a scalable and cost-efficient real2sim pipeline for neural 3D scene reconstruction and simulation. Given a monocular video as input, Vid2Sim can generate photorealistic and physically interactable 3D simulation environments to enable the reinforcement learning of visual navigation agents in complex urban environments. Extensive experiments demonstrate that Vid2Sim significantly improves the performance of urban navigation in the digital twins and real world by 31.2% and 68.3% in success rate compared with agents trained with prior simulation methods.

==> figtex/teaser.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/teaser-v5-compressed.pdf}
    \vspace{-2mm}
     \captionof{figure}{\ourmodel can convert monocular videos captured by hand-held camera into realistic and interactive simulation environments. It facilitates RL training of embodied navigation agents in digital twins and provides realistic observations to reduce the Sim-to-Real gap.
     % \TODO{Get a new realworld for Bottom-right image with 1. no laptop on the top 2. more complex settings}
     }
    \label{fig:teaser}
    \vspace{-2mm}
\end{figure*}
